Large-momentum-transfer atom interferometers with $\mu$rad-accuracy using Bragg diffraction

Large-momentum-transfer~(LMT) atom interferometers using elastic Bragg scattering on light waves are among the most precise quantum sensors to date. To advance their accuracy from the mrad to the $\mu$rad regime, it is necessary to understand the rich phenomenology of the Bragg interferometer, which differs significantly from that of a standard two-mode interferometer. We develop an analytic model for the interferometer signal and demonstrate its accuracy using comprehensive numerical simulations. Our analytic treatment allows the determination of the atomic projection noise limit of an LMT Bragg interferometer, and provides the means to saturate this limit. It affords accurate knowledge of the systematic phase errors as well as their suppression by two orders of magnitude down to a few $\mu\mathrm{rad}$ using appropriate light pulse parameters.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
